Facial Video-based Remote Physiological Measurement via Self-supervised Learning

Facial video-based remote physiological measurement aims to estimate remote photoplethysmography (rPPG) signals from human face videos and then measure multiple vital signs (e.g. heart rate, respiration frequency) from rPPG signals. Recent approaches achieve it by training deep neural networks, which normally require abundant facial videos and synchronously recorded photoplethysmography (PPG) signals for supervision. However, the collection of these annotated corpora is not easy in practice. In this paper, we introduce a novel frequency-inspired self-supervised framework that learns to estimate rPPG signals from facial videos without the need of ground truth PPG signals. Given a video sample, we first augment it into multiple positive/negative samples which contain similar/dissimilar signal frequencies to the original one. Specifically, positive samples are generated using spatial augmentation. Negative samples are generated via a learnable frequency augmentation module, which performs non-linear signal frequency transformation on the input without excessively changing its visual appearance. Next, we introduce a local rPPG expert aggregation module to estimate rPPG signals from augmented samples. It encodes complementary pulsation information from different face regions and aggregate them into one rPPG prediction. Finally, we propose a series of frequency-inspired losses, i.e. frequency contrastive loss, frequency ratio consistency loss, and cross-video frequency agreement loss, for the optimization of estimated rPPG signals from multiple augmented video samples and across temporally neighboring video samples. We conduct rPPG-based heart rate, heart rate variability and respiration frequency estimation on four standard benchmarks. The experimental results demonstrate that our method improves the state of the art by a large margin.

==> sec/4_theory.tex <==
\section{Theory analysis}
For the sake of simplicity, we suppose each periodic rPPG signal can be represented as a periodic trigonometric function, \ie $y=A\sin (2\pi F (t+\varphi))$. $A$, $F$ and $\varphi$ respectively denotes the signal amplitude, frequency and shift. Thus, to increase/decrease its frequency by a factor of $f$, \ie to obtain signal $\hat{y}=A\sin (2\pi fF (t+\varphi))+B$, $y$ should be multiplied with another modulation signal $\hat{f}$. We take $f=2$ as an example, and $\hat{f}$ should be:
\begin{equation}\label{equ5}
    \begin{split}
    \hat{f}= A\sin (4\pi F (t+\varphi))/A\sin (2\pi F (t+\varphi))\\
    =\sin (4\pi F (t+\varphi))/\sin (2\pi F (t+\varphi))\\
    =\cos (2\pi F (t+\varphi))
    \end{split}
\end{equation}
which also contains information ($F$, $\varphi$) from $y$. In other words, this modulation signal is determined by the original rPPG signal $y$ and the target frequency ratio $f$. We realize this process by two 1D RB and a BiLSTM layer in the proposed frequency modulation block (FMB) of FAM. 1D RB layers and BiLSTM layer respectively perform local and global signal transformation and frequency error correction. The combination of nonlinear activation functions (ReLU, Sigmoid and Tanh) in these layers are beneficial to achieve the corresponding nonlinear transformation. After obtaining the modulation signal, we multiply it with the original rPPG signal to change the frequency of latter.
